The Monocular Depth Estimation Challenge

This paper summarizes the results of the first Monocular Depth Estimation Challenge (MDEC) organized at WACV2023. This challenge evaluated the progress of self-supervised monocular depth estimation on the challenging SYNS-Patches dataset. The challenge was organized on CodaLab and received submissions from 4 valid teams. Participants were provided a devkit containing updated reference implementations for 16 State-of-the-Art algorithms and 4 novel techniques. The threshold for acceptance for novel techniques was to outperform every one of the 16 SotA baselines. All participants outperformed the baseline in traditional metrics such as MAE or AbsRel. However, pointcloud reconstruction metrics were challenging to improve upon. We found predictions were characterized by interpolation artefacts at object boundaries and errors in relative object positioning. We hope this challenge is a valuable contribution to the community and encourage authors to participate in future editions.

==> Figures/res_depth_viz.tex <==
% SYNS-Patches Depth Visualizations

\scriptsize

\def\first{0127}
\def\nums{0431, 0571, 0715}
\def\dataset{SynsDepth}

\def\methods{
    img/
    ,gt/GT
    ,jspenmar/Baseline
    ,hwscut/\teamone
    ,zsuri/\teamtwo
    ,yiyiyihahaha/\teamthree
    ,Team/\teamfour
}

\foreach \method/\label in \methods{%
    \begin{tikzpicture}[every node/.style={inner sep=0,outer sep=0,anchor=south west}]
        \node (image) at (0, 0) {\includegraphics[width=0.23\linewidth]{\dataset/\method_\first.png}};
        \begin{scope}[x={(image.south east)},y={(image.north west)}]
            \draw (0.01, 0.01) node {\textbf{\label}};
        \end{scope}
    \end{tikzpicture}
    %
    \foreach \num in \nums{%
        \includegraphics[width=0.23\linewidth]{\dataset/\method_\num.png}
    } \\
}

\mycaption{\acl{syns} Depth Visualization}{%
Models perform significantly better in urban environments that resemble the training automotive data. 
Thin structures, such as the railings and branches, are highly challenging to predict accurately and are commonly merged together. 
}


==> Figures/syns.tex <==
% SYNS-Patches Sample Images

\foreach \img in {img, depth, edges}{%
    \foreach \num in {07_07, 08_03, 16_06, 29_01}{%
        \includegraphics[width=0.24\linewidth]{Syns/\img_\num.png}
    } \\
}
\vspace{0.1cm}
\foreach \img in {img, depth, edges}{%
    \foreach \num in {31_12, 47_01, 82_08, 87_17}{%
        \includegraphics[width=0.24\linewidth]{Syns/\img_\num.png}
    } \\
}

\mycaption{\acl{syns} Challenge Dataset}{%
We show some representative examples from the diverse set of testing categories. 
This includes complex urban, natural and indoor scenes with high-quality dense \acs{lidar}.
Depth boundaries were computed as Canny edges in the log-depth maps. 
}


==> Tables/datasets.tex <==
% Dataset Statistics

\mycaption{Dataset \& Benchmark Comparison}{%
We summarize recent datasets commonly used in self-supervised monocular depth estimation. 
CityScapes represents a common pretraining dataset, while \acl{syns} is testing-only.
\acl{syns} is the only dataset providing high-quality dense depth maps in a wide variety of environments.
}

\begin{tabular}{llllllllll}
\toprule
                                                  &    Accuracy & Density (\%) &  Num Points &  Urban & Natural &  Indoor &   Train &     Val &    Test \\
\midrule
                     CityScapes~\cite{Cordts2016} &      \xmark &       \xmark &      \xmark & \cmark &  \xmark &  \xmark &  88,250 &  \xmark &  \xmark \\
      Kitti Eigen-Zhou~\cite{Geiger2013,Zhou2017} &      \xmark &       \xmark &      \xmark & \cmark &  \xmark &  \xmark &  39,810 &   4,424 &  \xmark \\
\midrule
          Kitti Eigen~\cite{Geiger2013,Eigen2015} &         Mid &         4.10 &         19k & \cmark &  \xmark &  \xmark &  45,200 &   1,776 &     697 \\
Kitti Eigen-Benchmark~\cite{Geiger2013,Uhrig2018} &        High &        15.28 &         71k & \cmark &  \xmark &  \xmark &  71,633 &   5,915 &     652 \\
                        DDAD~\cite{Guizilini2020} &        High &         1.02 &         24k & \cmark &  \xmark &  \xmark &  75,900 &  23,700 &   3,080 \\
\midrule
          \acl{syns}~\cite{Adams2016,Spencer2022} &        High &        78.30 &        365k & \cmark &  \cmark &  \cmark &  \xmark &     400 &     775 \\
\bottomrule
\end{tabular}


==> Tables/res_metrics.tex <==
% SYNS-Patches Results


\mycaption{\acl{syns} Results}{%
Each sections reports results over a different set of scene categories. 
The updated \ac{sota} models from~\cite{Spencer2022} provide a strong baseline for the challenge, outperforming all submissions in pointcloud reconstruction F-Score.
However, all submissions significantly improved upon traditional image-based metrics by up to 6.47\% in MAE and 7.42\% in AbsRel. 
All approaches adapt better to unseen outdoor urban environments that the challenging natural and agricultural scenes. 
}

\begin{tabular}{@{}lllllllll@{}}
\toprule
                                           &            &    F-Score\up & F-Score (Edges)\up &     MAE\down &     RMSE\down &   AbsRel\down &  EdgeAcc\down &  EdgeComp\down \\ 
\midrule           
             \multirow{5}*{\emph{Overall}} &   Baseline &  \best{13.72} &        \best{7.76} &         5.56 &          9.72 &         32.04 &          3.97 &   \best{21.63} \\
                    \cline{2-9}
                                           &   \teamone & \nbest{13.53} &               7.41 &  \best{5.20} &  \nbest{8.98} &  \best{29.66} &  \nbest{3.67} &  \nbest{27.31} \\
                                           &   \teamtwo &         13.08 &               7.46 &         5.39 &          9.27 &         29.96 &          3.81 &          32.70 \\
                                           & \teamthree &         12.85 &               7.30 &         5.32 &          9.04 &         30.22 &          3.83 &          43.77 \\
                                           &  \teamfour &         12.66 &       \nbest{7.51} & \nbest{5.22} &   \best{8.96} & \nbest{29.70} &   \best{3.36} &          35.47 \\
\midrule
       \multirow{5}*{\emph{Outdoor-Urban}} &   Baseline &  \best{14.09} &        \best{6.48} &         4.77 &          8.43 &         29.10 &          3.89 &   \best{22.75} \\ 
       \cline{2-9}   
                                           &   \teamone & \nbest{13.17} &       \nbest{5.99} &  \best{4.53} &  \nbest{7.93} &  \best{27.12} &  \nbest{3.47} &  \nbest{27.71} \\ 
                                           &   \teamtwo &         12.72 &               5.97 &         4.77 &          8.25 &         27.99 &          3.64 &          34.31 \\ 
                                           & \teamthree &         12.83 &               5.56 &         4.60 &          7.95 &         28.04 &          3.66 &          41.04 \\ 
                                           &  \teamfour &         12.00 &               5.87 & \nbest{4.54} &   \best{7.85} & \nbest{27.91} &   \best{3.12} &          35.24 \\ 
\midrule   
     \multirow{5}*{\emph{Outdoor-Natural}} &   Baseline &  \best{12.11} &       \nbest{5.32} &         7.46 &          12.86 &         36.89 &          3.84 &   \best{18.35} \\
     \cline{2-9}   
                                           &   \teamone &         11.61 &               5.26 &  \best{6.82} &   \best{11.52} & \nbest{33.53} &  \nbest{3.52} &  \nbest{24.11} \\
                                           &   \teamtwo &         11.40 &               5.25 &         7.14 &          12.07 &         34.43 &          3.61 &          30.96 \\
                                           & \teamthree &         11.83 &               5.31 &         7.11 &          11.76 &         34.16 &          3.59 &          38.96 \\
                                           &  \teamfour & \nbest{11.84} &        \best{5.72} & \nbest{6.92} &  \nbest{11.72} &  \best{33.33} &   \best{3.30} &          31.33 \\
\midrule   
 \multirow{5}*{\emph{Outdoor-Agriculture}} &   Baseline & \nbest{12.26} &        \best{4.77} &         6.10 &          10.84 &         33.58 &          4.00 &   \best{18.73} \\ 
 \cline{2-9}   
                                           &   \teamone &         12.26 &               4.47 & \nbest{5.78} &          10.20 &         31.53 &  \nbest{3.69} &  \nbest{27.38} \\ 
                                           &   \teamtwo &  \best{12.75} &               4.40 &         5.85 &          10.33 &  \best{30.52} &          3.77 &          29.03 \\ 
                                           & \teamthree &         11.53 &               4.20 &         5.78 &  \nbest{10.12} & \nbest{30.76} &          3.87 &          41.89 \\ 
                                           &  \teamfour &         11.34 &       \nbest{4.57} &  \best{5.72} &   \best{10.03} &         30.99 &   \best{3.40} &          33.53 \\ 
\midrule   
             \multirow{5}*{\emph{Indoor}}  &   Baseline & \nbest{21.11} &       \best{28.96} &         1.04 &          1.51 &         22.77 &  \nbest{4.60} &  \nbest{37.09} \\ 
             \cline{2-9}   
                                           &   \teamone &  \best{23.56} &              27.95 & \nbest{1.00} &          1.54 &  \best{21.12} &          4.82 &   \best{36.28} \\ 
                                           &   \teamtwo &         19.95 &      \nbest{28.84} &  \best{0.98} &   \best{1.42} &         21.44 &          5.20 &          43.93 \\ 
                                           & \teamthree &         19.32 &              28.82 &         1.07 &          1.55 &         23.94 &          5.10 &          74.43 \\ 
                                           &  \teamfour &         20.45 &              27.65 &         1.01 &  \nbest{1.49} & \nbest{21.16} &   \best{4.28} &          55.52 \\ 
\bottomrule
\end{tabular}


==> Tables/syns_cat.tex <==

% SYNS-Patches Category Distribution

\mycaption{\acl{syns} Category Distribution}{}

\begin{tabular}{@{}llllllllll|l@{}}
\toprule
               & Agriculture & Indoor & Industry & Misc & Natural & Recreation & Residential & Transport & Woodland & Total \\ 
\midrule
  \textbf{Val} &         104 &     67 &       36 &   72 &      36 &         14 &          13 &         4 &       54 &   400 \\ 

 \textbf{Test} &         211 &     81 &       71 &    0 &     147 &         48 &         110 &        17 &       90 &   775 \\ 
\midrule
\textbf{Total} &         315 &    148 &      107 &   72 &     183 &         62 &         123 &        21 &      144 & 1,175 \\ 
\bottomrule
\end{tabular}

